Mitigating Test-Time Bias for Fair Image Retrieval

We address the challenge of generating fair and unbiased image retrieval results given neutral textual queries (with no explicit gender or race connotations), while maintaining the utility (performance) of the underlying vision-language (VL) model. Previous methods aim to disentangle learned representations of images and text queries from gender and racial characteristics. However, we show these are inadequate at alleviating bias for the desired equal representation result, as there usually exists test-time bias in the target retrieval set. So motivated, we introduce a straightforward technique, Post-hoc Bias Mitigation (PBM), that post-processes the outputs from the pre-trained vision-language model. We evaluate our algorithm on real-world image search datasets, Occupation 1 and 2, as well as two large-scale image-text datasets, MS-COCO and Flickr30k. Our approach achieves the lowest bias, compared with various existing bias-mitigation methods, in text-based image retrieval result while maintaining satisfactory retrieval performance. The source code is publicly available at \url{https://anonymous.4open.science/r/Fair_Text_based_Image_Retrieval-D8B2}.

==> chapters/2_related_works.tex <==
\section{Related work} 
\label{sec:rel_works}
% image retrieval using VL models 
% 整合 fairness in machine learning + VL 
% 偏 HCI 的介绍 user perception 

\paragraph{Text-based image retrieval}
Text-based image retrieval is the process of searching and retrieving images from a large database using textual descriptions or keywords as queries.
The task is usually tackled by image-text feature alignment~\citep{cao2022image}, which embeds image and text inputs into a shared feature space such that relevant image and text features are close to each other.
In recent years, substantial progress has been made due to the emergence of large-scale datasets, as well as the development of effective deep learning-based image-text models.
Pioneering works include DeViSE~\citep{frome2013devise}, which bridges the {\em semantic gap} between image content and textual descriptors by aligning CNN-based features of images with textual embeddings from ImageNet labels.
Subsequent approaches, such as VSE++~\citep{faghri2017vse++} and SCAN~\citep{lee2018stacked}, further refine these joint embeddings to improve retrieval performance.
%
Recently, OpenAI's CLIP~\citep{radford2021learning} has emerged as a powerful approach for image retrieval based on similarity matching between extracted image and text features.
CLIP leverages a pre-trained transformer model, jointly optimized for both image and text understanding, which allows it to effectively match images and textual descriptions.
On challenging zero-shot image retrieval tasks, CLIP has outperformed many traditional supervised fine-tuned models~\citep{radford2021learning}.

\vspace{-2mm}
\paragraph{Fairness in machine learning}
Recent studies have highlighted numerous unfair behaviors in machine learning models~\citep{angwin2016machine, buolamwini2018gender}.
For example, a risk assessment algorithm used in the United States criminal justice system predicted that Black defendants were more likely to commit future crimes than white defendants, even after controlling for criminal record~\citep{angwin2016machine}.
Moreover, individuals with different gender and skin-tones are likely to receive disparate treatment in commercial classification systems such as Face++, Microsoft, and IBM systems~\citep{buolamwini2018gender}.
Consequently, there has been a surge in demand and interest for developing methods to mitigate bias, such as regularizing disparate impact~\citep{zafar2015learning} and disparate treatment~\citep{hardt2016equality}, promoting fairness through causal inference~\citep{kusner2017counterfactual}, and incorporating fairness guarantees in recommendations and information retrieval~\citep{beutel2019fairness, morik2020controlling}. 

\vspace{-2mm}
\paragraph{Fairness in vision-language models}
After some studies revealed the bias of using VL models in downstream tasks~\citep{wang2021gender, hall2023vision, wang2021assessing}, efforts to address and mitigate these biases in VL models have gained increasing attention.
Existing solutions for fair vision-language models can be generally classified into pre-processing, in-processing, and post-processing methods.
Pre-processing techniques usually involve re-weighting or adjusting the training data to counter imbalances across demographic attributes, while preserving the utility of the dataset for the target task~\citep{friedler2014certifying, calmon2017optimized}.
%\rh{you have not defined protected group}.
In-processing methods focus on altering the training objective by incorporating fairness constraints, regularization terms or leveraging adversarial learning to obtain representations invariant to gender/race~\citep{berg2022prompt,wang2023toward, xu2021robust, cotter2019optimization}.
Post-processing approaches achieve fairness by applying {\em post-hoc} corrections to a (pre-)trained model~\citep{cheng2021fairfil, calmon2017optimized} or via feature clipping~\citep{wang2021gender} on the output of image-text encoders based on mutual information. 

Our work lies in the post-processing category of debiasing methods that encourages equal representation of diverse demographics.
We also identified the fair subset selection approach used in \citet{mehrotra2021mitigating} as a potential post-hoc debiasing method for TBIR.
While \citet{mehrotra2021mitigating} shares our goal of ensuring equality of gender/race attributes in the set of results, their focus did not extend to the TBIR scenario with an underlying VL model nor detail an effective method for obtaining accurate demographic attributes for debiasing.
More importantly, they assumed demographic attributes seen by their algorithm to be available ground truth labels subject to noise.
This assumption creates difficulties when attempting to adapt their method to a real-world problem such as TBIR.
Complementary, our approach is meant to address these deficiencies by providing a practical debiasing procedure, that includes acquiring demographic attributes.


%We have identified a post-processing methods with the potential to address our target task 
% \rh{you say several, but below only one is mentioned}.
% We also identify a post-hoc fair subset selection approach~\citep{mehrotra2021mitigating} with potential to reduce bias in our TBIR using CLIP.
% Specifically, FairExpec selects a subset from candidate pools, where the subset maximize the utility scores(can be similarity score in TBIR), while constraining the number of demographic attributes of individuals selected to the subsets.
%FairExpec solves the problem of maximum target sum of the utility of individuals while constraining the number of demographic attributes included in the selected subset \rh{rephrase, what is fairexpec? what is number of demographics? sum of what?}.
% The sum is computed with the utility of each individual, such as their similarity to a query, while the constraint pertains to the noisy demographic attributes of each individual 
% \rh{this sentence makes no sense}.
% Though \citet{mehrotra2021mitigating} laid the groundwork with FairExpec, their focus did not extend to the TBIR context with an underlying VL model or detail an effective method for obtaining accurate demographic attributes for debiasing. Moreover, in their assumptions, they only allow demographic attributes to be ground truths with noises, presenting challenges of adapting FairExpec to real-world problem such as TBIR. Our approach is meant to address these deficiencies by providing a comprehensive and applicable pipeline for post-hoc debiasing in TBIR. \rh{how?}.
% Some similar post-processing methods have been explored in fair subset selection and fair ranking~\citep{mehrotra2021mitigating, mehrotra2022fair}, in the way that they select the subset of images or re-rank the image list based on provided utilities and gender/race representation scores 
% \rh{what is utility in this context? they select them or re-rank them for what purpose?}.

% \rh{what about the methods in the other two references? what do you mean by ``does not work''? what is a probability vector?}. 
%\rh{How is your method differentto FairExpec? Do you only consider one baseline? if so, why? if not, you need to mention them here and why yours is different to them}

% \WT{In terms of pre-trained models' bias calibration, I think our current method falls into the post-processing category, because 1) we didn't touch the pre-training data, 2) we didn't touch the pre-training itself}

% \WT{1) Is ranking a general category of bias calibration method? Or do you just want to mention fairness issues in the ranking technique? }

% \paragraph{Fairness in Vision-Language Models} 
% In recent literature, there has been an increasing focus on addressing biases in multimodal settings.
% For example, \citep{agarwal2021evaluating} and \citep{wang2021gender} have proposed methods to mitigate gender bias in CLIP embeddings by removing dimensions that exhibit strong correlations with gender attributes.
% Moreover, \citep{berg2022prompt} have contributed by debiasing CLIP models through prompt learning, utilizing an adversarial approach.
% \citep{zhang2022contrastive} have also addressed the issue of group robustness in vision-language models, employing contrastive learning techniques \rh{what is group robustness?}.

% Notably, these prior works have largely focused on debiasing models by modifying the weights of the model, which is prohibitive when the model weights are not public, or the model is too large to re-train.
% adopted data-oriented strategies, relying on the training or fine-tuning of models using labeled datasets \rh{disconnected sentence}. 

% \paragraph{Gender/Racial Bias in Web Image Search}
% % \fj{add bias about dataset, images, and their captions}
% Our work is closely related to studies in the Human Computer Interaction community that demonstrated gender inequality in online image search results~\citep{kay2015unequal}.
% These studies revealed how gender bias in occupational image search results influences people's perceptions about gender in various professions.
% Moreover, investigations into racial bias in search results, such as those conducted by \citet{noble2018algorithms}, have shown that these biases can reinforce harmful stereotypes and contribute to the perpetuation of systemic inequalities.
% % \rh{here stereotype seems to be used differently}.
% % For example, when searching for terms like ``successful person'' or ``professional hairstyles'', the results might predominantly return images of white individuals, inadvertently excluding individuals of color.
% Notable biases across different demographic subgroups are present in image search results, even when using neutral queries such as ``smiling''~\citep{celis2020implicit}.
% Importantly, these biases can shape user perceptions and further amplify existing biases.
% Our work builds upon these findings by examining the gender and racial bias in text-based image retrieval algorithm and offering an innovative solution for reducing bias in popular image retrieval framework using pre-trained VL model, such as CLIP~\citep{radford2021learning}.

